A review of path following control strategies for autonomous robotic vehicles: theory, simulations, and experiments

This article presents an in-depth review of the topic of path following for autonomous robotic vehicles, with a specific focus on vehicle motion in two dimensional space (2D). From a control system standpoint, path following can be formulated as the problem of stabilizing a path following error system that describes the dynamics of position and possibly orientation errors of a vehicle with respect to a path, with the errors defined in an appropriate reference frame. In spite of the large variety of path following methods described in the literature we show that, in principle, most of them can be categorized in two groups: stabilization of the path following error system expressed either in the vehicle's body frame or in a frame attached to a "reference point" moving along the path, such as a Frenet-Serret (F-S) frame or a Parallel Transport (P-T) frame. With this observation, we provide a unified formulation that is simple but general enough to cover many methods available in the literature. We then discuss the advantages and disadvantages of each method, comparing them from the design and implementation standpoint. We further show experimental results of the path following methods obtained from field trials testing with under-actuated and fully-actuated autonomous marine vehicles. In addition, we introduce open-source Matlab and Gazebo/ROS simulation toolboxes that are helpful in testing path following methods prior to their integration in the combined guidance, navigation, and control systems of autonomous vehicles.

==> ABSTRACT.tex <==
 This article presents an in-depth review on the topic of path following of autonomous vehicles in two dimensional space (2D). From a control system standpoint, path following can be formulated as a stabilization problem of the path following error system that describes the dynamics of position and orientation errors between a vehicle and a pre-assigned path, defined in an appropriate reference frame. Although there is a large variety of path following methods described in the literature we show that, in principle, most of them can be categorized in two groups: either stabilization of the path following error system in the vehicle's body frame or in a frame attached to a \emph{``reference point"} moving along the path, such as a Frenet–Serret (F-S) frame or a Parallel Transport (P-T) frame. With this observation, we provide a unified formulation that is simple but general enough to cover many methods available in the literature. We then discuss the advantages and disadvantages of each method, comparing them from the design and implementation standpoint. We further show experimental results of the path following methods obtained from field trials testing with under-actuated and fully-actuated autonomous marine vehicles. Finally, we introduce Matlab and Gazebo/ROS simulation toolboxes that are helpful in testing the path following methods and integrating them in guidance navigation and control systems.  

==> Experimental_results.tex <==
% -*- root:Main_survey.tex -*-
{
\color{black}
\section{Experimental results} \label{sec: experiement}
In this section, we report the results of field trials aimed at assessing the performance of the path following algorithms described previously for an autonomous surface vehicle. 
\subsection{Test set-up}
The fields tests were conducted with two Medusa class autonomous surface vehicles built at IST. The first one is an under-actuated Medusa shown in Fig.\ref{fig: underactuated vehicles}. This type of vehicle has played central roles in many European research projects such as Morph\cite{PedroMorph} and Wimust \cite{PedroWimust} to support the research in marine science and also in the area of guidance, navigation and control of single and networked multiple autonomous vehicle. The under-actuated Medusa vehicle is equipped with two starboard and portside thrusters that allow for the generation of longitudinal forces and torques about the vertical axis. path following methods. The second Medusa that was used in the trial is fully-actuated that is shown in Fig.\ref{fig: fully actuated-vehicle}. This vehicle contain six thrusters. Two thrusters are mounted vertically and four thrusters are mounted horizontally. The thruster configuration in the fully actuated vehicle allows for the generation of longitudinal and lateral forces and torque about the vertical axis. \\
The two vehicles' navigation system builds upon GPS-RTK and AHRS sensors that allow for the computation of its position and orientation. All software modules for navigation and control were implemented using the Robot Operating System (ROS, Melodic version), programmed with C++, and ran on an EPIC computer board (model NANO-PVD5251). More information about the specification of the Medusa class vehicle can be found in \cite{abreu2016medusa}. The implementation of the path following controllers follows the structure depicted in Fig. \ref{fig: path following system}. The vehicle's inner-loop controllers include three proportional integrator and derivative (PID)-type controllers to track the references in linear speed, heading, and heading rate that are generated by the path following controllers. \\
The trials were conducted at a lake next to Expo'98, Lisbon, Portugal. Snapshots showing the vehicle performing path following can be seen in Fig.\ref{fig: medusa at trials} while its operation can be monitored online with a console shown in \ref{fig:console}. 
\begin{figure}
	\centering
	\includegraphics[width=.47\textwidth]{pictures/Medusa_red_working.jpg} \hfill
	\includegraphics[width=.47\textwidth]{pictures/yellow_at_sea.JPG} \vfill
	a) Under-actuated Medusa           \hspace{80pt}          b) Fully-actuated Medusa  
	\caption{The vehicles performing path following during the trial}
	\label{fig: medusa at trials}
\end{figure} 
\begin{figure}[h!]
	\centering
	\includegraphics[trim=0.0cm 0.0cm 0.0cm 0cm,width=0.9\linewidth,clip]{pictures/console.png} 
	\caption{Console to operate the Medusa class vehicles}
	\label{fig:console}
\end{figure}
%In order to test the path following method, we 
%\textcolor{red}{We will insert 3 pictures here: 1 - Medusa on land , 2 - Medusa at water, 3 - Console (performing Bernoulli path). Anyone has those (fresh) images? if yes, please send them to me.}
\subsection{Results}
\subsubsection{Result with the under-actuated vehicle}
As shown in Fig. \ref{fig:position_lawnmower}, during the tests the vehicles followed assigned paths consisting of lawnmowing paths with a first leg of $30m$ heading north, then a half circumference turning anticlockwise with a radius of $10m$, a second leg of $20m$ heading south,  another half circumference with a radius of $10m$ turning clockwise, and a final leg of $30m$ heading north. In another set of tests the vehicles were made to follow a Bernoulli lemniscate with a length of $20m$ as shown in \ref{fig:position_bernouli}. In all the tests, the assigned speed of the vehicles $U_{\rm d}$ is $0.5m/s$. During the trials were tested the \emph{Method} 1-4, 6, and the method in \cite{Pramod2009}.

Figures \ref{fig:position_lawnmower} and \ref{fig:position_bernouli} show the paths of the vehicles during the trials for the different methods. We observe that the vehicles follow their assigned paths and that the transient behavior and tracking performance vary according to the method used.

\begin{figure}[h!]
	\centering
	\includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=0.7\linewidth,clip]{PF_results/position_lawnmower.pdf} 
	\caption{Vehicle paths using different methods during experiments performing path following of lawnmowing maneuvers.  Filled circles are initial position of the vehicle.}
	\label{fig:position_lawnmower}
\end{figure}

\begin{figure}[hbt!]
	\centering
\includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=0.7\linewidth,clip]{PF_results/position_bernouli.pdf} 
	\caption{Vehicle paths using different methods during experiments aimed at testing path following of a Bernoulli lemniscate. Filled circles are initial position of the vehicle}
	\label{fig:position_bernouli}
\end{figure}

The \emph{cross-track} errors $y_1$ (defined in Section \ref{section: derivation of path following error in path frame}) of the vehicles performing a lawnmowing maneuver using different path following methods is shown in Figure \ref{fig:cross_track_lawnmower}. Identical results for the case where the path is a Bernoulli lemniscate are shown in \ref{fig:cross_track_bernouli}.
\begin{figure}[htb!]
\centering
\begin{minipage}{.5\textwidth}
  \captionsetup{width=.9\linewidth}
  \centering
  \includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=\linewidth,clip]{PF_results/cross_track_lawnmower.pdf} 
  \captionof{figure}{\emph{Cross-track} errors for different methods while performing lawnmower maneuvers.}
  \label{fig:cross_track_lawnmower}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \captionsetup{width=.9\linewidth}
  \includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=\linewidth,clip]{PF_results/cross_track_bernouli.pdf} 
  \captionof{figure}{\emph{Cross-track} errors for different methods while describing a Bernoulli lemniscate.}
  \label{fig:cross_track_bernouli}
\end{minipage}
\end{figure}
From figures \ref{fig:cross_track_lawnmower} and \ref{fig:cross_track_bernouli} one can observe that \emph{Method 3-4} took less time to converge than the other methods. \\
The \emph{along-track} errors $s_1$, defined in Section \ref{section: derivation of path following error in path frame}, of the vehicles performing the lawnmower missions is shown in Figure \ref{fig:along_track_lawnmower} and following the Bernoulli lemniscate in \ref{fig:cross_track_bernouli}. Figures \ref{fig:along_track_lawnmower}-\ref{fig:along_track_bernnouli} show data for \emph{Method 2}, 4 and 6 since for all the other methods the ``\emph{reference point}'' is the orthogonal projection of the vehicle's position on the path so the \emph{along-track} error is always zero.
\begin{figure}[htb!]
\centering
\begin{minipage}{.5\textwidth}
  \captionsetup{width=.9\linewidth}
  \centering
  \includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=\linewidth,clip]{PF_results/along_track_lawnmower.pdf} 
  \captionof{figure}{\emph{Along-track}  errors for different methods while performing lawnmower maneuvers.}
  \label{fig:along_track_lawnmower}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \captionsetup{width=.9\linewidth}
  \centering
  \includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=\linewidth,clip]{PF_results/along_track_bernouli.pdf} 
  \captionof{figure}{\emph{Along-track} errors for different methods while describing a Bernoulli lemniscate.}
  \label{fig:along_track_bernnouli}
\end{minipage}
\end{figure}

From Figures \ref{fig:along_track_lawnmower}-\ref{fig:cross_track_bernouli} one can observe that the along track error converges to close to zero for \emph{Method 2} and 4 and for \emph{Method 6} stabilizes at $1m$ due to the effect of $\bs \epsilon$ on the particular definition of the position error \ref{eq: eB}. We can also observe, for the Bernoulli lemniscate mission with \emph{Method 6}, large oscillations at the beginning. However, these oscillations have little impact on the behavior of the vehicle given the large distance to the ``\emph{reference point}''.

Figures \ref{fig:surge_speed_lawnmower} and \ref{fig:surge_speed_bernouli} show the surge speed $u$ of the vehicle for different methods for the lawnmower and Bernoulli lemniscate missions respectively, which clearly indicate that the vehicle asymptotically reaches the desired constant speed profile (0.5m/s). However they show that the surge speed converged faster to the desired speed for \emph{Method} 3, 4 and the Method in \cite{Pramod2009}.
%\pagebreak

\begin{figure}[htb!]
\centering
\begin{minipage}{.5\textwidth}
  \captionsetup{width=.9\linewidth}
  \centering
  \includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=\linewidth,clip]{PF_results/surge_speed_lawnmower.pdf} 
  \captionof{figure}{Surge speed for different methods while performing lawnmower maneuvers.}
  \label{fig:surge_speed_lawnmower}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \captionsetup{width=.9\linewidth}
  \centering
  \includegraphics[trim=1.5cm 7.5cm 1.5cm 8cm,width=\linewidth,clip]{PF_results/surge_speed_bernouli.pdf} 
  \captionof{figure}{Surge speed for different methods while describing a Bernoulli lemniscate.}
  \label{fig:surge_speed_bernouli}
\end{minipage}
\end{figure}

\subsubsection{Results with the fully-actuated vehicle}
The method for fully actuated vehicles in Section \ref{sec: fully actuated} was tested with a fully actuated Medusa class vehicle following a line due east (along the $Y$ axis) with a heading $\psi$ of $0^{\circ}$. The results are shown in Figure \ref{fig:position_fully_actuated}.

\begin{figure}[hbt!]
	\centering
	\includegraphics[trim=0cm 7cm 0cm 7.5cm,width=0.6\linewidth,clip]{PF_results/free_heading.pdf} 
	\caption{Vehicle trajectory using the method described in Section \ref{sec: fully actuated}. The initial positions of the vehicle is at (0,0).}
	\label{fig:position_fully_actuated}
\end{figure}

Given the coupling between surge, sway and yaw rate in the dynamics of the vehicle, the tunning of the PID inner loops of the real vehicle is a challenging task and we were not able to obtain adequate performance of circular maneuvers during the field trials. In Fig. \ref{fig:position_fully_actuated_sim} we show a the results of a Gazebo simulation of the vehicle, after further tuning of the inner-loops and path-following parameters, performing a lawnmower maneuver with a yaw reference of $45^{\circ}$ relative to the path tangent.

\begin{figure}[hbt!]
	\centering
	\includegraphics[trim=0cm 7cm 0cm 7.5cm,width=0.7\linewidth,clip]{free_heading_2.pdf} 
	\caption{Vehicle trajectory using the method described in Section \ref{sec: fully actuated}. The initial positions of the vehicle is at (0,0).}
	\label{fig:position_fully_actuated_sim}
\end{figure}
}







==> Guidance_in_3D.tex <==
\section{3D path following methods} \label{sec: pf in 3D}
 \subsection{Stabilizing path following error in path frames  }
 \subsubsection{Method 1: Achieve path following by controlling $(u,r,q,\dot{\gamma})$}
 \subsubsection{Method 2: Achieve path following by controlling $(u,\psi,\theta,\dot{\gamma})$}
 \subsubsection{Method 3: Light-of-Sight path following methods}
 
 \subsection{Stabilizing path following error in the vehicle's body frame }
  \subsubsection{Method 4: Achieve path following by controlling $(u,r,q,\ddot{\gamma})$}
 \subsection{Extension to external disturbances and robustness issues}
 

==> H_mathdefs.tex <==
\newcommand{\pfi}{\rm pf}
\newcommand{\abs}[1]{|#1|}														% Absolute of a scalar
\newcommand{\Enorm}[1]{{ \left\| {#1} \right\|}}						        % Euclide norm of a vector
\newcommand{\Inorm}[1]{{ \left\| \bf{#1} \right\|}_{\infty}}                    % Infinity norm of a vector
\newcommand{\Mnorm}[1]{{ \left\| #1 \right\|}}                                  % Matrix norm
\newcommand{\limin}[1]{\lim_{t\rightarrow\infty}{#1}} 						    % lim (t-> infinity)%
\newcommand{\bs}[1]{\boldsymbol{#1}}										    % bold symbol%					
\newcommand{\pard}[2]{\frac{\partial #1}{\partial #2}}     					    % partial derivative%
\newcommand{\origin}{\bs{x} =\bs{0}}
\newcommand{\xt}{\bs{x}(t)}
\newcommand{\ut}{{\bf{u}}(t)}
\newcommand{\x}{{\bf x}}
\newcommand{\xto}{{\bf x}(t_{0})}
\newcommand{\Wx}[1]{W_{#1}({\bf x})}
\newcommand{\alphax}[1]{\alpha_{#1}({\bf x})}
\newcommand{\alphanormx}[1]{\alpha_{#1}(\Enorm{x})}
\newcommand{\Vx}{V({ \bf x})}
\newcommand{\Vtx}{V(t,\bs{x})}
\newcommand{\fx}{\bs{f}({\bs x})}
\newcommand{\ftx}{\bs{f}(t,{\bs x})}
\newcommand{\fxu}{{\bf f}({\bf x},{\bf u})}
\newcommand{\ftxu}{\bs{f}(t,\bs{x},\bs{u})}
\newcommand{\dotx}[1]{{\dot{\bf{x}}}_{#1}}
\newcommand{\ftxc}[2]{\bs{f}_{#1}(t,\bs{x}_{#2})}
\newcommand{\gtxc}[2]{\bs{g}_{#1}(t,\bs{x}_{#2})}
\newcommand{\normU}{{ \left\|U\right\|}}						        % Euclide norm of a vector
%\newcommand{\dev}[2]{ \frac { d#1 }{ dt } }}

%----- Symbol of Sets-----------------------------
\newcommand{\compl}{\mathbb{C}}         
\newcommand{\real}{\mathbb{R}}
\newcommand{\realnon}{{\mathbb{R}_{0}^{+}}}
\newcommand{\Ka}{\mathcal K}
\newcommand{\La}{\mathcal L}
\newcommand{\N}{\mathbb{N}}
%------End of Symbol of Set-----------------------
%------Symbol of General vector r-----------------
\newcommand{\vecr}{\boldsymbol{r}}
\newcommand{\vecomega}{\boldsymbol{\omega}}         
\newcommand{\dvecr}{\left( \frac { d\boldsymbol{r} }{ dt }  \right) }
\newcommand{\dvec}[2]{\left( \frac { d\boldsymbol{#1}_{#2} }{ dt }  \right) }
\newcommand{\dvecnormal}[1]{\left( \frac { d{#1} }{ dt }  \right)}
\newcommand{\colcomvecr}[1]{\left[ \begin{matrix} { {x_{#1} }} \\ { {y_{#1}}} \end{matrix} \right] }
\newcommand{\rowcomvecr}[1]{\left[ \begin{matrix} { {x_{#1} }} & { {y_{#1}}} \end{matrix} \right] }
\newcommand{\colcomvecrxyz}[1]{\left[ \begin{matrix} { {x_{#1} }} \\ { {y_{#1}}} \\{ {z_{#1}}}\end{matrix} \right] }
\newcommand{\coldotcomvecr}[1]{\left[ \begin{matrix} { {\dot{x_{#1}} }} \\ { {\dot{y_{#1}}}} \end{matrix} \right] }
\newcommand{\rowdotcomvecr}[1]{\left[ \begin{matrix} { {\dot{x_{#1}} }} & { {\dot{y_{#1}}}} \end{matrix} \right] }
\newcommand{\coltwo}[2]{\left[ \begin{matrix}  #1 \\ #2 \end{matrix} \right] }
\newcommand{\colfour}[4]{\left[ \begin{matrix}  #1 \\ #2 \\ #3 \\#4 \end{matrix} \right] }

 
%\newcommand{\K}{{\boldsymbol{k}}}
%------End of Symbol of General Vector------------
%------Symbol in Reference frame {I}---------------
\newcommand{\iI}{{\boldsymbol{i}}_{ I }}
\newcommand{\jI}{{\boldsymbol{j}}_{ I }}
\newcommand{\kI}{{\boldsymbol{k}}_{ I }}
%\newcommand{\xI}{{x_{I}}}
%\newcommand{\yI}{{y_{I}}}
\newcommand{\zI}{z_{\mathcal{I}}}
\newcommand{\dxI}{\left( \frac { d{ {x_{I}} }  }{ dt }  \right) }
\newcommand{\dyI}{\left( \frac { d{ {y_{I}} }  }{ dt }  \right) }
\newcommand{\dzI}{\left( \frac { d{ {z_{I}} }  }{ dt }  \right) }
\newcommand{\vecIP}{\overrightarrow { IP } }
\newcommand{\dvecIP}{\left(\frac{d\overrightarrow { IP }}{dt}\right)}
\newcommand{\vecrIP}{{\boldsymbol{r}}_{P/I}}
\newcommand{\dvecrIP}{\left(\frac{d\vecrIP}{dt}\right)}
\newcommand{\vecIB}{\overrightarrow { IB } }
\newcommand{\vecrIB}{{\boldsymbol{r}}_{B/I}}
\newcommand{\basisI}{{\boldsymbol{i} }_{ I }, { \boldsymbol{j} }_{ I },{\boldsymbol{k} }_{ I }} 
\newcommand{\basisIinxy}{{\boldsymbol{i} }_{ I }, { \boldsymbol{j} }_{ I }} 
\newcommand{\vecbasisI}{\left[ \begin{matrix}  {\boldsymbol{i} }_{ I } \\ { \boldsymbol{j} }_{ I }\\{\boldsymbol{k} }_{ I } \end{matrix} \right]}
\newcommand{\vecbasisIinxy}{\left[ \begin{matrix}  {\boldsymbol{i} }_{ I } \\ { \boldsymbol{j} }_{ I }\end{matrix} \right]}
\newcommand{\vPinI}{{\boldsymbol{ v }}_{P/I}}
\newcommand{\dvPinI}{\left(\frac{d\vPinI}{dt}\right)}
\newcommand{\aPinI}{{\boldsymbol{ a }}_{P/I}}
\newcommand{\vBinI}{{\boldsymbol{ v }}_{B/I}}
\newcommand{\dvBinI}{\left(\frac{d\vBinI}{dt}\right)}
\newcommand{\aBinI}{{\boldsymbol{ a }}_{B/I}}
%------End of Symbol in Reference frame {I}---------
%------Symbol in Reference frame {B}----------------
%\newcommand{\xB}{x_{B}}
%\newcommand{\yB}{y_{B}}
\newcommand{\zB}{z_{B}}
\newcommand{\dxB}{\left( \frac { d{ {x_{B}} }  }{ dt }  \right) }
\newcommand{\dyB}{\left( \frac { d{ {y_{B}} }  }{ dt }  \right) }
\newcommand{\dzB}{\left( \frac { d{ {z_{B}} }  }{ dt }  \right) }
\newcommand{\iB}{{\boldsymbol{i}}_{ B }}
\newcommand{\jB}{{\boldsymbol{j}}_{ B }}
\newcommand{\kB}{{\boldsymbol{k}}_{ B }}
\newcommand{\diB}{{ \left( \frac { d{\boldsymbol{i}}_{ B } }{ dt }  \right)  }}
\newcommand{\djB}{{ \left( \frac { d{\boldsymbol{j}}_{ B } }{ dt }  \right)  }}
\newcommand{\dkB}{{ \left( \frac { d{\boldsymbol{k}}_{ B } }{ dt }  \right)  }}
\newcommand{\basisB}{{\boldsymbol{i} }_{ B }, { \boldsymbol{j} }_{ B },{\boldsymbol{k} }_{ B }}
\newcommand{\basisBinxy}{{\boldsymbol{i} }_{ B }, { \boldsymbol{j} }_{ B }}
\newcommand{\vecbasisB}{\left[ \begin{matrix}  {\boldsymbol{i} }_{ B } \\ { \boldsymbol{j} }_{ B } \\ {\boldsymbol{k} }_{ B } \end{matrix} \right]} 
\newcommand{\vecbasisBinxy}{\left[ \begin{matrix}  {\boldsymbol{i} }_{ B } \\ { \boldsymbol{j} }_{ B } \end{matrix} \right]} 
\newcommand{\vecBP}{\overrightarrow { BP } } 
\newcommand{\vecrBP}{{\boldsymbol{r}}_{P/B}}
\newcommand{\vPinB}{{\boldsymbol { v }}_{P/B}}
\newcommand{\aPinB}{{\boldsymbol{a}}_{P/B}}
%-----End of Symbol in Reference Frame {B}--------------
%-----Symbol of transformation matrix----------------------------
\newcommand{\RBtoI}{{ R }_{ B }^{ I }}
\newcommand{\RItoB}{{ R }_{ I }^{ B }}
\newcommand{\matBtoI}{\left[ \begin{matrix} \cos\theta  & -\sin\theta  \\ \sin\theta  & \cos\theta  \end{matrix} \right]}
\newcommand{\matItoB}{\left[ \begin{matrix} \cos\theta  &  \sin\theta  \\ -\sin\theta  & \cos\theta  \end{matrix} \right]}
\newcommand{\dotmatBtoI}{\dot{\theta}\left[\begin{matrix} -\sin\theta & -\cos\theta\\\cos\theta  & -\sin\theta \end{matrix}\right]}
\newcommand{\Matrix}[1]{\left[\begin{matrix}#1\end{matrix}\right]}


%% Notation in frames
\newcommand{\F}{\mathcal{F}}							% in Frenet frame 
\newcommand{\B}{\mathcal{B}}							% in Body frame
\newcommand{\I}{\mathcal{I}}							% in Inertial frame
\newcommand{\Fframe}{\left\{ \mathcal{F} \right\}} 	% Frenet frame
\newcommand{\Iframe}{\left\{ \mathcal{I} \right\}} 	% Inertial frame
\newcommand{\Bframe}{\left\{ \mathcal{B} \right\}} 	% Body frame
\newcommand{\xI}{x_{\I}}							    % in Frenet frame 
\newcommand{\yI}{y_{\I}}							    % in Frenet frame 
\newcommand{\xB}{x_{\B}}							    % in Frenet frame 
\newcommand{\yB}{x_{\B}}							    % in Frenet frame 
\newcommand{\xF}{x_{\F}}							    % in Frenet frame 
\newcommand{\yF}{x_{\F}}							    % in Frenet frame 
\newcommand{\ef}{{\bf e}_{\F}}                           % error vector in Frenet frame 
\newcommand{\ddef}{\dot{\ef}}
\newcommand{\exf}{e_{x}}								% x component of error vector in Frenet frame	
\newcommand{\exfi}{{e^{[i]}_{x}}}					    % x component of error vector in Frenet frame	
\newcommand{\eyf}{e_{y}}								% x component of error vector in Frenet frame
\newcommand{\eyfi}{{e^{[i]}_{y}}}								% x component of error vector in Frenet frame
\newcommand{\dexf}{\dot{e}_{x}}
\newcommand{\deyf}{\dot{e}_{y}}	
\newcommand{\psiF}{\psi_{\F}}                           % angle of Frenet frame
\newcommand{\psie}{\psi_{e}}
\newcommand{\psiei}{\psi^{[i]}_{e}}
\newcommand{\RItoF}{{ R }_{ \I }^{ \F }}
\newcommand{\RFtoI}{{ R }_{ \F }^{ \I }}
\newcommand{\matItoF}{\left[ \begin{matrix} \cos\psiF  & \sin\psiF & 0 \\ -\sin\psiF  & \cos\psiF  & 0 \\ 0 & 0 & 1  \end{matrix} \right]}
\newcommand{\p}{{\bf p}}
\newcommand{\pd}{{\bf p}_{\rm d}}
\newcommand{\pdi}{{\bf p}^{[i]}_{\rm d}}
\newcommand{\psii}{\psi^{[i]}}
\newcommand{\psidi}{\psi^{[i]}_{\rm d}}
\newcommand{\ri}{r^{[i]}}
%% 
\newcommand{\rf}{r_{\F}}
\newcommand{\rd}{r_{\rm d}}
\newcommand{\psid}{\psi_{\rm d}}
\newcommand{\dpsid}{\dot{\psi}_{\rm d}}
\newcommand{\rchi}{r_{\chi}}
\newcommand{\cur}{\kappa(s)}
\newcommand{\curg}{\kappa(\gamma)}
\newcommand{\curgi}{\kappa^{[i]}(\gammai)}
%% Dynamics in frames
\newcommand{\dpI}{\left( \frac { d{ {\p} }  }{ dt }  \right)_{\I} }
\newcommand{\dpF}{\left( \frac { d{ {\p} }  }{ dt }  \right)_{\F} }
\newcommand{\dpdF}{\left( \frac { d{ {\pd} }  }{ dt }  \right)_{\F} }
\newcommand{\dpdI}{\left( \frac { d{ {\pd} }  }{ dt }  \right)_{\I} }
\newcommand{\deff}{\left( \frac { d{ {\ef} }  }{ dt }  \right)_{\F} }
\newcommand{\ds}{\dot{s}}
\newcommand{\dx}{\dot{x}}
\newcommand{\dxi}{\dot{x}^{[i]}}
\newcommand{\dy}{\dot{y}}
\newcommand{\dyi}{\dot{y}^{[i]}}
\newcommand{\dpsi}{\dot{\psi}}
\newcommand{\dpsii}{\dot{\psi}^{[i]}}
\newcommand{\dchi}{\dot{\chi}}
\newcommand{\dpsie}{\dot{\psie}}
\newcommand{\vcx}{v_{\rm cx}}
\newcommand{\vcy}{v_{\rm cy}}
\newcommand{\hatvcxy}{\hat{\bs{v}}_{cxy}}
\newcommand{\dhatvcxy}{\dot{\hat{\bs{v}}}_{cxy}}
%% Path notation
\newcommand{\Path}{\mathcal{P}}
\newcommand{\vds}{v_{\rm d}(s)}
\newcommand{\vd}{v_{\rm d}}
%\newcommand{\u1}{u_{1}}
%\newcommand{\u2}{u_{2}}
%\newcommand{\u}{\bs{u}}
\newcommand{\xbar}{{\bar{\bf x}}}
\newcommand{\xbari}{{\bar{\bf x}}^{[i]}}
\newcommand{\dxbari}{{\dot{\xbar}}^{[i]}}
\newcommand{\e}{{\bf e}}
\newcommand{\f}{ {\bf f} }
\renewcommand{\u}{{\bf u}}
\newcommand{\ubar}{\bar{\bf u}}
\newcommand{\ubari}{{\bar{\bf u}}^{[i]}}

\newcommand{\ebar}[1]{\bar{\bf e}#1}
\newcommand{\debar}{\dot{\bar{\bs{e}}}}
\newcommand{\depfbar}{\dot{\bar{\e}}_{\pfi}}
\newcommand{\dbargamma}{\dot{\bar{\gamma}}}
\newcommand{\dbargammai}{\dot{\bar{\gamma}}^{[i]}}
\newcommand{\dbargammaj}{\dot{\bar{\gamma}}^{[j]}}
\newcommand{\Upf}{\mathbb{U}_{\rm pf}}
\newcommand{\Ucpf}{\mathbb{U}_{\rm cpf}}
\newcommand{\Upfi}{\mathbb{U}^{[i]}_{\rm pf}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\vcxy}{\bs{v}_{cxy}}
\newcommand{\phat}{\hat{\bs{p}}}
\newcommand{\ur}{u_{\rm r}}
\newcommand{\dur}{\dot{u}_{\rm r}}
\newcommand{\vr}{v_{\rm r}}
\newcommand{\dvr}{\dot{v}_{\rm r}}
\newcommand{\ep}{\bs{e}_{p}}
\newcommand{\ec}{\bs{e}_{c}}
\newcommand{\matrixtwo}[4]{\left[ \begin{matrix} & #1 & #2 \\ & #3 & #4  \end{matrix}   \right]}
\newcommand{\OCPI}{\mathcal{OCP}_{1}(t,\x^{[i]}(t),\gammai(t), \gammaj(t),T_{\rm p})}
\newcommand{\OCPII}{\mathcal{OCP}_{2}(t,\x^{[i]}(t),\gammai(t), \gammaj(t),T_{\rm p})}
\newcommand{\rootsquare}{\sqrt{U^2-\Enorm{\vc}^2\sin^{2}(\alpha-\psi)}}   
\newcommand{\vb}{{\bf v}_{\rm b}}
\newcommand{\vc}{{\bf v}_{\rm c}}
\newcommand{\Tp}{T_{\rm p}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ISUnit
\newcommand{\mps}{\si{\meter \per \second}}
\newcommand{\rps}{\si{\radian \per \second}}
\newcommand{\mpone}{\si{\meter^{-1}}}
\newcommand{\dpsiF}{\dot{\psi}_{\mathcal{F}}}
\newcommand{\umpcI}{{\bf u}_{\rm mpc1}}
\newcommand{\umpcII}{{\bf u}_{\rm mpc2}}
\newcommand{\vecs}[3]{{\bf #1}_{#2}^{#3}}
\renewcommand{\vec}[1]{{\bf #1}}
\newcommand{\ua}{\vecs{u}{\rm a}{}}

% graph theorey
\newcommand{\G}{\mathcal{G}}
\newcommand{\vertex}{\mathcal{V}}
\newcommand{\edge}{\mathcal{E}}
\newcommand{\neigbor}{\mathcal{N}}

\newcommand{\epf}{{\bf e}_{\rm pf}}
\newcommand{\epfi}{{\bf e}^{[i]}_{\rm pf}}
\newcommand{\depfi}{\dot{{\bf e}}^{[i]}_{\rm pf}}
\newcommand{\dg}{\dot{\gamma}}
\newcommand{\upf}{{\bf u}_{\rm pf}}
\newcommand{\upfi}{{\bf u}^{[i]}_{\rm pf}}
\newcommand{\upfbar}{\bar{\bf u}_{{\rm pf}i}}
\newcommand{\epfbar}{\bar{\bf e}_{{\rm pf}i}}

\newcommand{\vci}{v^{[i]}_{\rm c}}
\newcommand{\vcbari}{ \bar{v}^{[i]}_{\rm c}}
\newcommand{\vi}{v^{[i]}}
\newcommand{\urmax}{u_{\rm r_{\max}}}
\newcommand{\Ni}{\mathcal{N}_{i}}  
\newcommand{\Lvd}{L_{v_{\rm d}}}
\newcommand{\xd}{x_{\rm d}}
\newcommand{\yd}{y_{\rm d}}
\newcommand{\Ug}{\U_{\dg}}
\newcommand{\ith}{i^{\rm th}}
\newcommand{\jth}{j^{\rm th}}
\newcommand{\gammai}{\gamma^{[i]}}
\newcommand{\hatgammaii}{\hat{\gamma}^{[ii]}}
\newcommand{\hatgammaij}{\hat{\gamma}^{[ij]}}
\newcommand{\hatgammaji}{\hat{\gamma}^{[ji]}}
\newcommand{\gammaj}{\gamma^{[j]}}
\newcommand{\gammaN}{\gamma^{[N]}}
\newcommand{\dgammai}{\dot{\gamma}^{[i]}}
\newcommand{\tki}{t_{i,k}}
\newcommand{\tkj}{t_{j,k}}
\newcommand{\tkij}{t_{ij,k}}

\newcommand{\ui}{u^{[i]}}
\newcommand{\dsi}{\dot{s}^{[i]}}
\newcommand{\Ri}{R^{[i]}}
\newcommand{\xit}{{\bf x}^{[i]}}
\newcommand{\Ji}{J^{[i]}}
\newcommand{\li}{l^{[i]}}
\newcommand{\uai}{{\bf u}^{[i]}_{\rm a}}
\newcommand{\ubi}{{\bf u}^{[i]}_{\rm b}}
\newcommand{\bargammai}{\bar{\gamma}^{[i]}}
\newcommand{\bargammaj}{\bar{\gamma}^{[j]}}
\newcommand{\minus}{\text{-}}
%\newcommand{\fi}{{\bf f}^{[i]}}
 
\newcommand{\R}{\mathbb{R}}

%%%%%%%%%%%%%%%% Graph theory
\newcommand{\Nin}{\Ni^{\rm in}}
\newcommand{\Nout}{\Ni^{\rm out}}
\newcommand{\Din}{D^{\rm in}}
\newcommand{\Dout}{D^{\rm out}}
\newcommand{\din}{d^{\rm in}_i}
\newcommand{\dout}{d^{\rm out}_i}
\newcommand{\dtau}{{\rm d} \tau}
\newcommand{\h}{ {\bf h}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\rmT}{{\rm T}}
\newcommand{\subscript}[1]{\scriptscriptstyle{#1}}
\newcommand{\eB}{\e_{\subscript{\B}}}
\newcommand{\eP}{\e_{\subscript{\mathcal{P}}}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\RPI}{R^{\subscript{\mathcal{I}}}_{\subscript{\mathcal{P}}}}
\newcommand{\RIP}{R^{\subscript{\mathcal{P}}}_{\subscript{\mathcal{I}}}}
\newcommand{\RBI}{R^{\subscript{\mathcal{I}}}_{\subscript{\mathcal{B}}}}
\newcommand{\RIB}{R^{\subscript{\mathcal{B}}}_{\subscript{\mathcal{I}}}}
\newcommand{\rmB}{\subscript{\mathcal{B}}}
\newcommand{\rmP}{\subscript{\mathcal{P}}}	
\newcommand{\OCP}{\mathcal{OCP}}
	

==> NOTATION.tex <==
\section{Preliminaries} \label{sec: notation and background}

\textcolor{red}{I will think more to see if it is necessary to have this section or not as the reference frames and other notation already described in section 3. I am also thinking to put the next lemma in Appendix rather than here.}  \\~\\
%\subsection{Notation}
%In what follows, we let $\R,\R_{>0},$ and $\R_{\ge 0}$ denote the set of real, positive real, and nonnegative real numbers, respectively. We shall use the notation $\Enorm{\cdot}$ to denote the Euclidean norm of a vector in $ \R^n$. Given matrices
%$A, B \in \R^{n\times n}$ the notation $A \succeq B$ means that $A − B$ is
%positive semi-definite. Given $\x\in \R^{n}$ and $Q\in \R^{n\times n } , \Enorm{\x}_{Q}\triangleq \x^{\rm T}Q\x$.  
%	Given $x,y \in \R$, Young's inequality states that, for any $a \in \R_{>0}$, 
%	\begin{equation} \label{eq: Young's inequality}
%	xy \le \frac{ax^{2}}{2}+ \frac{y^{2}}{2a}.
%	\end{equation}
%A continuous function $\alpha: [0,a)\to[0,\infty)$ is said to be of class $\Ka$ if it is strictly increasing and $\alpha(0)=0$ and of class $\Ka_{\infty}$ if $a=\infty$ and $\alpha(r)\to\infty$ as $r\to\infty$. A continuous function $\beta: [0,a)\times[0,\infty) \to[0,\infty)$ is said to be of class $\Ka \La$ if, for each fixed $s$, the mapping $\beta(r,s)$ is of class $\Ka$ with respect to $r$ and, for each fixed $r$, the mapping $\beta(r,s)$ is decreasing with respect to $s$ and $\beta(r,s)\to 0$ as $s\to\infty$.
 The following lemma will be used in the paper.
%\begin{definition}
%	content...
%\end{definition}
\begin{lemma}[Rotation Matrix Differential Equation, Theorem 2.2 \cite{fossen2011handbook}]
	Let $R^{B}_{A} \in SO(n)$\footnote{A special orthogonal group in dimension $n$, defined as $SO(n)=\{ R\in \R^{n\times n}: RR^{\rm T}=R^{\rm T} R=I_n, \det{R}=1  \}$ }$(n=2,3)$ be the rotation matrix from frame $\{A\}$ to frame $\{B\}$. Then,
\begin{equation} \label{eq: Rotation DE}
\dot{R}^{ B}_{A}={R}^{ B}_{A}S(\bs{\omega}^{A}_{A/B}),
\end{equation}	
 where $S(\bs{\omega}^{A}_{A/B})$ is a Skew-symmetric matrix\footnote{A square matrix $S$ is called a Skew-symmetric matrix iff $S^{\rm T}=-S$.} and $\bs{\omega}^{A}_{A/B}\in \R^{n} $ is the angular velocity vector of $\{A\}$ respect to $\{B\}$, expressed in $\{A\}$.	
\end{lemma}
%Example: Let ${\bs \omega} = [q,p,r] \in \R^3$ be the angular velocity of the vehicle body frame $\mathcal{B}$ respect to an inertial frame $\Iframe$ , expressed $\mathcal{B}$    
% Given a symmetric matrix $A$, the symbols ${\lambda_{\min}}(A)$ and ${ {\lambda}_{\max}}(A)$ denote the smallest and the largest eigenvalues of $A$. Given vectors $\x_i\in \R^{n}; i=1,...,N$, ${\rm col}(\x_1,...,\x_N)\triangleq [\x^{\rm T}_1,...,\x^{\rm T}_N]^{\rm T}\in \R^{n\times N} $. The notation $\N({\bs \mu},P)$ denotes a Gaussian (normal) distribution with mean $\bs{\mu}$ and covariance matrix $P$.
% 
 % \begin{lemma} \label{lemma: Fischer lemma}
 % 	\textit{
 % 		Let $L$ be the Laplacian matrix of a weight-balanced and strongly connected digraph $\G$. Then, 0 is a simple eigenvalue of $L_s$ and, for any $\x \in \R^{N}$ such that $\x\perp\bf {1}$, the following inequalities hold:
 % 		$$
 % 		\lambda_2(L_s)\Enorm{\x}^{2} \le \x^{\rm T}L_s\x \le \lambda_N(L_s)\Enorm{\x}^{2},  
 % 		$$
 % 		where $\lambda_{2}(L_s)$ and $\lambda_{N}(L_s) \in \R_{>0} $ are the second smallest and the largest eigenvalues of $L_s$, respectively.
 % 	}
 % \end{lemma} 
 % \textit{Proof:} Since $L_s$ is symmetric and {\bf 1} is the eigenvector associated with the eigenvalue 0, the inequality follows from the Courant-Fischer theorem in \cite{horn1990matrix}. \hfill $\blacksquare$
 % \begin{lemma}[Finsler's lemma,\cite{boyd1994linear}]
 % \textit{
 % 	Given $A \in \R^{n}, B\in \R^{n\times m}$. The following LMI problems are equivalent: 
 % 	\begin{enumerate}[i.]
 % \item	$\exists  P\succ \bs{0}$ and $Y\in \R^{m\times n}$ s.t. $AP+PA^{\rm T}+BY+Y^{\rm T}B^{\rm T} \prec \bs{0} $
 % \item  $  \exists P\succ \bs{0}$ and $\tau\in \R$ s.t. $AP+PA^{\rm T}-\tau BB^{\rm T} \prec \bs{0} $
 % 	\end{enumerate}
 % }
 %\end{lemma}
 
 	%	where r and R are defined as in Lemma 3. Then, a(L) > 0. For balanced
 	
 	%	graphs, a(L) = λ2( L+ 2LT ), where λ2( L+ 2LT ) denotes the smallest nonzero
 	
 	%	eigenvalue of L+ 2LT .

==> PROBLEM_FORMULATION_3D.tex <==
\section{Problem formulation and common principles of path following methods} \label{sec: problem}
  \begin{figure}[h]
	\centering
	\includegraphics[width=90mm]{3D_illustration.pdf} 
	\caption{Geometry illustration of PF problem}
	\label{fig: 3D presentation}
\end{figure}~\\
Path following refers to the problem of making a vehicle converge to and follow a spatial path with a desired speed profile a long the path; see Fig. \ref{fig: 3D presentation}. To solve this problem, it requires a path following strategy that guide the motion of the vehicle in order to achieve path following. From a control system standpoint, a complete path following control system can be described as in Fig. \ref{fig: path following system}(a). In this architecture, the outer-loop path following controller plays the role of a guidance strategy, in charge of computing desired references (e.g. linear and angular speeds, or  orientations) to guide the vehicle to follow the path. These references are used as reference inputs for an autopilot which plays the role of an inner-loop controller, responsible for generating suitable forces and torque for the vehicle in order to track the desired references, and thereby achieve the path following objectives. \\
In practice, to simplify the design of a path following controller, it is commonly assumed that the responses of the autopilot and the vehicle dynamics (the inner-loop) are sufficiently fast so that the influence of the inner-loop in the complete system can be neglected, thus the path following control system can be simplified by considering the kinematics model as in Fig. \ref{fig: path following system}(b). Our purpose in the present paper is to review the core ideas behind path following methods, therefore we primarily focus on those designed for the vehicle kinematics only. We then treat the effect of the inner-loop as an internal disturbance and analyze the robustness of the path following methods under this disturbance accordingly. \\
The mathematical formulation of the path following problem for the vehicle kinematics is presented next.  
\begin{figure}[h]
	\centering
	\includegraphics[width=120mm]{Overall_Guidance.pdf} \\
	a) A complete path following control system ~\\~\\
	\includegraphics[width=120mm]{Simplified_PF_system.pdf} \\
	b) A simplified path following system for PF controller design
	\caption{Path following control systems. ${\bf u}_{\rm d}$: reference inputs (e.g. desired linear and angular speeds, orientations) for the autopilot,  $\p$ and $\bs{\eta}$: the vehicle's position and orientations, respectively. }
	\label{fig: path following system}
\end{figure}
\subsection{Vehicle kinematic models}
  \begin{figure}[h]
	\centering
	\includegraphics[width=90mm]{3D_illustration.pdf} 
	\caption{Geometry illustration of PF problem}
	\label{fig: 3D presentation}
\end{figure}
The vehicle's motion is illustrated Fig. \ref{fig: 3D presentation}. In what follows, $\{\I\} = \{x_\I, y_\I, z_\I\}$ denotes an inertial North-East-Down (NED) frame, where the axis $\xI$ points to the North, the axis $\yI$ points to the East,  and the axis $\zI$ points downward, normal to the Earth's surface. Let $Q$ be the center of mass of the vehicle and denote by ${\bf p}=[x, y, z]^{\rm T} \in \R^{3}$ the position of $Q$ in  $\Iframe$. Let also $\{\B\} = \{x_\B, y_\B, z_\B\}$ be a body-fixed frame whose origin is attached at $Q$. In addition, denote by ${\bf v}=[u,v,w]^{\rm T} \in \R^{3} $ the vehicle's velocity vector and $\bs{\omega}=[p,q,r]^{\rm T}\in \R^{\rm 3} $ the angular velocity, expressed in $\Bframe$. With the above notation, the vehicle' kinematic model is given by
\begin{subequations}
 \label{original tracker model}
\begin{align}
\dot{\p}&=\RBI({\bs \eta}){\bf v} , \\
\dot{\bs \eta}&=T(\bs \eta){\bs \omega },
%\dot{v}^{[i]}&=\Fi, \quad \dri =\tau^{[i]},
%\dyi&=\ui\sin\psii, \qquad \qquad  \dot{u}^{[i]}=F^{[i]}, \\	
%\dzi&=0,  \quad \quad  \qquad  \quad  \qquad\quad          \dot{r}^{[i]}=\tau^{[i]},
\end{align}
\end{subequations}
where according to Ch.2 \cite{fossen2011handbook} $\RBI({\bs \eta}) \in SO(3)$ is the rotation matrix from $\Bframe$ to $\Iframe$ and $T(\bs \eta)\in \R^{3\times 3} $ is a transformation matrix, locally parameterized by a vector ${\bs \eta}\triangleq[\phi,\theta,\psi]^{\rm T}$ that contains the Euler angles of roll $(\phi)$, pitch $(\theta)$ and yaw $(\psi)$, given by
%\begin{equation}
%\RBI(\bs{\eta})=R_{\rm z}(\psi)R_{\rm y}(\theta)R_{\rm x}(\phi)
%\end{equation}
\begin{equation} \label{eq: RBI and T}
\begin{aligned}
\RBI(\bs{\eta})&= \begin{bmatrix}
\rm c\psi c\theta & −\rm s\psi c\phi + \rm c\psi s \theta s \phi & \rm s\psi s\phi + \rm c\psi c\phi s\theta\\
\rm s \psi c\theta & \rm c\psi c\phi + s\phi s \theta s\psi & \rm −c\psi s\phi + s\theta s\psi c\phi\\
−\rm s\theta & \rm c\theta s\phi & \rm c\theta c\phi\\
\end{bmatrix}\\
T(\bs{\eta})&= \begin{bmatrix}
1 &  \rm s\phi t \theta &  \rm  c\phi t\theta\\
0 & \rm  c\phi & \rm −s\phi \\
0 & \rm s\phi/c\theta  & \rm c\phi/c\theta \\
\end{bmatrix},\\
\end{aligned}
\end{equation}
where $\rm s \cdot\triangleq \sin(\cdot), c\cdot\triangleq \cos(\cdot)$ and $\rm t\cdot\triangleq\tan(\cdot)$.
%with 
%\begin{equation}
%\begin{aligned}
%R_{\rm z}(\psi)&=\begin{bmatrix}
%\cos(\psi) & -\sin(\psi) & 0\\
%\sin(\psi) & \cos(\psi) & 0\\
%0 & 0 & 1\\
%\end{bmatrix}, R_{\rm z}(\psi)=\begin{bmatrix}
%\cos(\psi) & -\sin(\psi) & 0\\
%\sin(\psi) & \cos(\psi) & 0\\
%0 & 0 & 1\\
%\end{bmatrix},\\
% R_{\rm z}(\psi)&=\begin{bmatrix}
%\cos(\psi) & -\sin(\psi) & 0\\
%\sin(\psi) & \cos(\psi) & 0\\
%0 & 0 & 1\\
%\end{bmatrix}
%\end{aligned}
%\end{equation}
%
%
%. See complete expressions of the transformation matrices $\RBI(\bs{\eta})$ and $T(\bs{\eta})$ in Chapter 2 of \cite{fossen2011handbook}. 
For the simplicity in conveying the core ideas of path following methods we temporarily omit the effect of external disturbances such as ocean current or wind in the kinematic model. However, after presenting the path following methods for this model, we will revisit them under external disturbances.   \\
In the present paper, we consider path following methods for the class of under-actuated vehicles for which ${\bf v}=[u,0,0]^{\rm T}$ and ${\bs \omega}=[0, q, r]^{\rm T}$. In marine robotics, this implies that the heave and sway speeds are neglected and we can only manipulate the forward speed $(u)$, while the roll motion are neglected as well ($\phi(t) \equiv 0$). With the these assumptions, the kinematics model in \eqref{original tracker model} can be rewritten explicitly as \\
{\bf 3D - kinematics model:}
\begin{equation} \label{eq: kinematics in 3D}
\begin{split}
\dot{x}&=u\cos(\psi)\cos(\theta)                    \\
\dot{y}&=u\sin(\psi)\cos(\theta)					\\	
\dot{z}&=u\sin(\theta)					\\
\dot{\theta}&=q                    \\
\dot{\psi}&=r\cos^{-1}(\theta).					\\	
\end{split}
\end{equation} 
Furthermore, if the vehicle's motion is restricted in the $x_{\I}-y_{\I}$ horizontal plan (i.e. $z(t)\equiv	0$ and $\theta(t) \equiv 0 $) then the vehicle kinematics in \eqref{eq: kinematics in 3D} can be simplified as\\
{\bf 2D - kinematics model:}
\begin{equation} \label{eq: kinematics in 2D}
\begin{split}
\dot{x}&=u\cos(\psi) \\
\dot{y}&=u\sin(\psi)					\\
\dot{\psi}&=r.				
\end{split}
\end{equation}   
\begin{remark}
	The 3D kinematic model given by \eqref{eq: kinematics in 3D} is equivalent to the 3D kinematic model of fixed wing UAV studied in \cite{Isaac2010}. The main difference between this model and that in \cite{Isaac2010} are in the signs of equations for $\dot{y}$ and $\dot{z}$ which comes from on the differences in the coordinate conventions adopted for the inertial frames. 
\end{remark}
\begin{remark}
	The 2D kinematic model given by \eqref{eq: kinematics in 2D} is adequate for a large class of vehicles that include unicycle mobile robots \cite{Samson1993,lapierre2006nonsingular},  fixed-wing UAVs  undergoing planar motion \cite{rucco2015model}, and a wide class of under-actuated AMVs such as Medusa and Delfim \cite{abreu2016medusa} or Charlie \cite{ROB:ROB20303}, for which the sway speed is in practice so small that it can be neglected. A similar kinematic model with a drift term can be found in \cite{HungCAMS2018} for the case where the motion is disturbed by constant wind (for AUVs) or constant ocean current (for AMVs).
\end{remark}
\subsection{Path parameterization and path frames} \label{section: path frames}
Let $\mathcal{P}$ be a spatial path, defined in the inertial frame and parametrized by a scalar variable $\gamma$ (e.g. arc-length). For the 3D case, the position of a generic point $P$, denoted by $\pd$ on the path is given by  
\begin{equation} \label{eq: path in 3D}
 \pd(\gamma)=[x_{\rm d}(\gamma),y_{\rm d}(\gamma),z_{\rm d}(\gamma)]^{\rm T} \in \R^{3},
\end{equation}
whereas, for the 2D case the position of this point is described by
\begin{equation} \label{eq: path in 2D}
\pd(\gamma)=[x_{\rm d}(\gamma),y_{\rm d}(\gamma)]^{\rm T} \in \R^2.
\end{equation}
 At $P$, there are three frames adopted in the literature to formulate the path following problem, namely, \emph{ Frenet–Serret} (F-S) frame, \emph{Parallel Transport} (P-T) frame, and a \emph{``Path"} frame. These frames are described next.
 \subsubsection{Frenet–Serret frame}
 This frame is used in the path following method of \cite{Samson1993,Lapierre2003,Isaac07} and is defined as follows. Let 
 \begin{equation} \label{eq: frenet frame}
 {\bf t}(\gamma)=\frac{\pd'(\gamma)}{\Enorm{\pd'(\gamma)}}, \quad {\bf n}(\gamma)=\frac{{\bf t}'(\gamma)}{\Enorm{{\bf t} '(\gamma)}}, \quad {\bf b}(\gamma)={\bf t}(\gamma)\times {\bf n}(\gamma).
 \end{equation}
 be the basis vectors defining the S-F frame at the point $\pd(\gamma)$ where for every differentiable $\f(x)$, $\f'(x)\triangleq \partial \f(x)/\partial x$. Then these vectors respectively define the unit tangent, \emph{principle} unit normal, and binormal to the path at the point determined
 by $\gamma$. The curvature $\kappa(\gamma)$ and the torsion $\tau(\gamma)$ of the path at that point are given as 
 \begin{equation} \label{eq: curvature}
 \kappa(\gamma)=\Enorm{{\bf t}'(\gamma)}}, \quad \tau(\gamma)=\Enorm{{\bf b}'(\gamma)}.
 \end{equation} 
  \subsubsection{Parallel–Transport frame}
  This frame was used the first time in the path following method of \cite{Isaac2010}. Although the Serenet-Frenet frame was adopted earlier in formulating the path following problem, it is not well-defined when the path has a vanish second derivative. The P-T frame overcomes this limitation and is defined as follows \cite{Hanson95paralleltransport}. The P-T frame is formed by three orthogonal basic vectors: the tangent vector ${\bf t}(\gamma)$ given in \eqref{eq: frenet frame}, and two vectors ${\bf n}_1(\gamma)$ and  ${\bf n}_2(\gamma)$, defining a normal plane perpendicular to ${\bf t}(\gamma)$. While ${\bf t}(\gamma)$ is fixed, ${\bf n}_1(\gamma)$ and  ${\bf n}_2(\gamma)$ can be chosen to satisfy the frame equations
  \begin{equation}
  \begin{bmatrix}
  \frac{{\rm d} {\bf t}(\gamma) }{{\rm d}\gamma} \\
  \frac{{\rm d} {\bf n}_1(\gamma) }{{\rm d}\gamma}\\
  \frac{{\rm d} {\bf n}_2(\gamma) }{{\rm d}\gamma}
  \end{bmatrix} = \begin{bmatrix}
  0 & k_1(\gamma) & k_2(\gamma)\\
  -k_1(\gamma) & 0 &0\\
  -k_2(\gamma) & 0 & 0
  \end{bmatrix} \begin{bmatrix}
  {\bf t}(\gamma)\\
  {\bf n}_1(\gamma) \\
  {\bf n}_2(\gamma) 
  \end{bmatrix},
  \end{equation}
  where the parameters $k_1(\gamma)$ and $k_2(\gamma)$ are related to the polar
coordinates of curvature and torsion as       
  \begin{equation}
  \kappa(\gamma)=\left(k_1(\gamma)+k_2(\gamma)\right)^{1/2}, \quad \tau(\gamma)=\frac{{\rm d}}{{\rm d}\gamma}\left(\tan^{-1}\left(\frac{k_2(\gamma)}{k_1(\gamma)}\right)\right).
  \end{equation}
 The difference between the F-S frame and the P-T frame can be illustrated in Fig. \ref{fig: S-F and P-T frame presentation}. With the F-S frame the normal component will switch sign at inflection points, while the P-T frame has no such discontinuities. 
    \begin{figure}[h]
  	\centering
  	\includegraphics[width=90mm]{2D_illustration_SF.pdf} 
  	\caption{An illustration of Frenet frame $\{\mathcal{F}\}$ and Parallel Transport frame $\{\mathcal{P}\}$.}
  	\label{fig: S-F and P-T frame presentation}
  \end{figure}
  
 \subsubsection{Other path frames} 
 Another path frame was introduced in the path following strategy of \cite{Breivik2005}. This frame is similar to the P-T frame and is obtain by performing two consecutive elementary rotations on the inertial frame $\Iframe$. The first is to rotate the $\Iframe$ about the z-axis an angle 
 \begin{equation}
 \psi_{\rmP} = \arctan\left(\frac{y'_{\rm d}(\gamma)}{x'_{\rm d}(\gamma)}\right).
 \end{equation} 
Then the path frame is obtained by rotating the resulting immediate frame about the y-axis and angle 
\begin{equation}
\theta_{\rmP} = \arctan\left(\frac{z'_{\rm d}(\gamma)}{\left(x'_{\rm d}(\gamma) + x'_{\rm d}(\gamma) \right)^{1/2} }\right).
\end{equation}
\subsection{Path following problem - a statement} \label{section: path following problem statement}
{\bf Path following control problem}:  \textit{Consider the spatial path $\mathcal{P}$ described by \eqref{eq: path in 3D}/\eqref{eq: path in 2D} for the 3D/2D cases and the vehicle with the kinematics model described by \eqref{eq: kinematics in 3D}/\eqref{eq: kinematics in 2D} for the 3D/2D cases, derive a feedback control law for the vehicle's inputs $(u,\psi, \theta)/(u,q,r)$ for 3D or $(u,\psi)/(u,r)$ for 2D, and possibly for $\dot{\gamma}$ or $\ddot{\gamma}$ so as to fulfill the following tasks:
		\begin{enumerate}[i)]
			\item Geometric task: drive the position error $\e \triangleq \p - \p_{\rm d}$ s.t. 
\begin{equation} \label{eq: gemetric task}
\lim_{t\to \infty} \e(t)={\bf 0}.
\end{equation}
			\item Dynamic task: ensure that the vehicle's forward speed tracks a positive desired speed profile $u_{\rm d}=u_{\rm d}(\gamma,t)$, i.e. 
			\begin{equation} \label{eq: dynamic task}
         \lim_{t\to \infty} u(t)- u_{\rm d}(t) = 0.
			\end{equation}	
		\end{enumerate}
}
Let $u_{\rmP}$ be the speed of $P$ with respect to the inertial frame, then
\begin{equation} \label{eq: uP}
u_{\rmP}=\frac{\rm d{\p}_{\rm d}}{{\rm d} t}=\Enorm{\p'_{\rm d}(\gamma) }\dot{\gamma}.
\end{equation}
Once the vehicle achieved path following, both the vehicle and the point $P$ would move with the desired speed profile $u_{\rm d}$, i.e. $u=u_{\rmP}=u_{\rm d}$, therefore the dynamics task in \eqref{eq: dynamic task} is equivalent with 
\begin{equation} \label{eq: dynamic task for gamma}
\lim_{t\to \infty} \dot{\gamma}(t)- v_{\rm d}(\gamma,t) = 0,
\end{equation}	
where $v_{\rm d}$ is the desired speed profile for $\dot{\gamma}$, defined by
\begin{equation} \label{eq: vd}
v_{\rm d}(\gamma,t) \triangleq \frac{1}{\Enorm{\p'_{\rm d}(\gamma)}}u_{\rm d}(\gamma,t).
\end{equation}
In path following, the point $P$ on the path plays the role of a \emph{``reference point"} for the vehicle to track. This point can be chosen as the nearest point to the vehicle \cite{Samson1993}, i.e. the orthogonal projection of the vehicle on the path, or can be initialized arbitrarily anywhere on the path and then its evolution are controlled through $\dot{\gamma}$ \cite{Lapierre2003,Breivik2005} or $\ddot{\gamma}$ \cite{aguiar2007trajectory} to achieve the path following objectives. In the latter cases, $\dot{\gamma}$ or $\ddot{\gamma}$ are considered as the controlled input of the dynamics of the \emph{``reference point"}, giving an extra freedom in designing path following controllers.
\subsection{Common principles of path following methods}
%{\bf List of important papers:}\textcolor{red}{[Just for a note, will be deleted]}
%\begin{enumerate}[i)]
%	\item Samson 1993 (2D)
%	\item Encarnasao, \cite{Encarnacao2000}, extend Samson to 3D.
%	\item  Aguiar (2D,3D)
%	\item  Lappier (2D) extends the work of Samson
%	\item Issac \cite{Isaac2010} - extend the work in paper of Lapier to 3D
%	\item Breivik and Fossen \cite{Breivik2005} (2D,3D) - control heading
%	\item MPC Adrea (2D,3D) based on formulation of Aguiar  
%	\item MPC Hung2018, Frank Alowgger (2D) based on formulation in Lapier
%	\item Nelson 2007 - vector field (2D) \cite{Nelson2007}
%	\item Sujit \cite{Sujit2014}-survey in air
%	\item 3D \cite{Encarnacao2000}
%	\item LOS
%\end{enumerate}
%From a control system standpoint, the path following is equivalent to a stabilization problem of the position error $\e$ and the error in to zero. 
Although there is a variety of path following methods in the literature, most of them can be categorized as in Table \ref{tab: principle of path following method}. The first category is for those stabilizing the position error in a frame attached to a \emph{reference point} point moving a long the path (e.g. F-S or P-T frames) whereas, the second is for those stabilizing the position error in the vehicle's body frame. The origin of the first approach can be traced back to the work of \cite{Samson1993} addressing the path following problem of unicycle-type and two-steering-wheels mobile robot. The core idea in this work was then adopted to develop more advanced path following algorithms in \cite{Lapierre2003,YuMPC2015,HungCAMS2018}. Later, we shall see that Light-of-Sight (LOS), a well-known path following method and widely used in marinecraft \cite{FOSSEN2003} can be categorized in this group as well. The second approach was proposed by \cite{aguiar2007trajectory} and further developed in \cite{alessandretti2013trajectory} to handle the vehicle's constraints. 
\begin{table}[hbt!] 
	\centering
	\caption{Common principles of path following methods }
	\vspace{-20pt}
	%	\begin{center}
		\begin{minipage}{\textwidth}
	{\begin{tabular*}{32pc}{@{\extracolsep{\fill}}clcc@{}}\\ \toprule
    &  \multirow{2}{*}{ ${\bf u}$}	 &\multicolumn{2}{c}{\bf Principles}\\ 		  \cmidrule{3-4}
			&   & Stabilizing  $\e$ in path frames	& Stabilizing $\e$ in the body frame \\	\midrule
	\multirow{2}{*}{\bf 2D}		&$u,\psi$	& \cite{FOSSEN2003,Breivik2005}								&    						\\ 
			&$u,r$	    &  	\cite{Samson1993,Lapierre2003} \cite{YuMPC2015,HungCAMS2018}							&   	\cite{aguiar2007trajectory}\cite{alessandretti2013trajectory}					\\ \midrule
	\multirow{2}{*}{\bf 3D}		&$u,\theta,\psi$	&  	\cite{Breivik2005}								&   						\\ 
			&$u,q,r$	& 	\cite{Encarnacao2000,Isaac2010}							&   \cite{aguiar2007trajectory}\cite{alessandretti2013trajectory}							\\ \midrule 
	\end{tabular*}}{}
\end{minipage}
	%	\end{tabular}
	\label{tab: principle of path following method}
\end{table}
%\begin{table}[hbt!] 
%	\centering
%	\caption{Categories of path following methods }
%	\vspace{-20pt}
%	{\begin{tabular*}{32pc}{@{\extracolsep{\fill}}ccccc@{}}\\ \toprule
%			&  \multirow{2}{*}{ ${\bf u}$}	 &\multicolumn{3}{c}{\bf Principles}\\ 		  \cmidrule{3-5}
%			&   & Stabilizing $\e_{\subscript{\B}}$  	& Stabilizing  $\e_{\subscript{\mathcal{P}}}$ & LOS\footnote{text} \\	\midrule
%			\multirow{2}{*}{\bf 2D}		&$u,\psi$	& 							&    					\cite{Breivik2005}		\\ 
%			&$u,r$	    &  	\cite{aguiar2007trajectory}								&   	\cite{Lapierre2003}						\\ \midrule
%			\multirow{2}{*}{\bf 3D}		&$u,\theta,\psi$	&  									&   	\cite{Breivik2005}					\\ 
%			&$u,q,r$	& 	\cite{aguiar2007trajectory}							&   	\cite{Encarnacao2000,Isaac2010}						\\ \midrule 
%	\end{tabular*}}{}
%	%	\end{tabular}
%	\label{tab: minimum inter event time}
%\end{table}



==> format.tex <==
%
%\usepackage[utf8x]{inputenc}
\usepackage[utf8x]{inputenc}
\usepackage{relsize,enumerate}
\usepackage{amsmath,amsfonts} % Math packages
\usepackage{siunitx}
\usepackage{amstext}
\usepackage{amssymb}

\usepackage{algorithm} 
%\usepackage{algorithmic}  
\usepackage[noend]{algpseudocode}
%\usepackage[english]{babel}
\usepackage[english]{babel} % English language/hyphenation
%
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remarks}{Remarks}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{problem}{Problem}
\newtheorem{algoritm}{Alogrithm}
\newtheorem{condition}{Condition}
%
\numberwithin{figure}{section}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
%\usepackage{subfig}    
\usepackage{float}
\usepackage{epstopdf}
\epstopdfsetup{update} %
%
%\usepackage{cite}
\usepackage{upgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{fullpage}
%\usepackage[protrusion=true,expansion=true]{microtype} % Better typography
%\usepackage{amsmath,amsfonts,amsthm} % Math packages
%\usepackage[svgnames]{xcolor} % Enabling colors by their 'svgnames'
%\usepackage[hang, small,labelfont=bf,up,textfont=it,up]{caption} % Custom captions under/above floats in tables or figures
%\usepackage{booktabs} % Horizontal rules in tables
%\usepackage{fix-cm}	 % Custom font sizes - used for the initial letter in the document
%\usepackage{amsmath,amssymb,amsfonts,amscd}
%\usepackage{sectsty} % Enables custom section titles
%\allsectionsfont{\usefont{OT1}{phv}{b}{n}} % Change the font of all section commands

%\usepackage{fancyhdr} % Needed to define custom headers/footers
%\usepackage{lastpage} % Used to determine the number of pages in the document (for "Page X of Total")
%\usepackage{tikz}
%\usetikzlibrary{calc,patterns,angles,quotes}
%\usetikzlibrary{shapes.geometric, arrows}
%\usepackage[abs]{overpic}
%\usepackage{verbatim,color}

%\usepackage{adjustbox}
%\usepackage{lettrine} % Package to accentuate the first letter of the text
%\newcommand{\initial}[1]{ % Defines the command and style for the first letter
%\lettrine[lines=3,lhang=0.3,nindent=0em]{
%\color{DarkGoldenrod}
%{\textsf{#1}}}{}}
%---------------------------------------------------------------
%\usepackage{titling} % Allows custom title configuration
%
%\newcommand{\HorRule}{\color{DarkGoldenrod} \rule{\linewidth}{1pt}} % Defines the gold horizontal rule around the title
%
% 

%\usepackage{bm}

%\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
%\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
%\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
%\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
%\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
%\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
%\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
%\makeatother

%---------------------------------------------------------------
%\usepackage{enumitem}
%\usepackage{cleveref}
%\usepackage{subfig}
%\DeclareMathOperator*{\minimize}{minimize}
%\typeout{pdfcompresslevel=\the\pdfcompresslevel}
%\typeout{pdfobjcompresslevel=\the\pdfobjcompresslevel}
%\typeout{pdfminorversion=\the\pdfminorversion}
%\pdfcompresslevel=9
%\pdfminorversion=5
%\pdfobjcompresslevel=2






%
%\usepackage{relsize,enumerate}
%%\usepackage{fullpage}
%\usepackage[english]{babel} % English language/hyphenation
%%\usepackage[protrusion=true,expansion=true]{microtype} % Better typography
%\usepackage{amsmath,amsfonts} % Math packages
%\usepackage{siunitx}
%\usepackage{amstext}
%\usepackage{upgreek}
%\usepackage{bm} 
%\usepackage{lipsum}
%\usepackage{tabularx}
%
%%\usepackage{amsmath,amsfonts,amsthm} % Math packages
%%\usepackage[svgnames]{xcolor} % Enabling colors by their 'svgnames'
%%\usepackage[hang, small,labelfont=bf,up,textfont=it,up]{caption} % Custom captions under/above floats in tables or figures
%%\usepackage{booktabs} % Horizontal rules in tables
%%\usepackage{fix-cm}	 % Custom font sizes - used for the initial letter in the document
%%\usepackage{amsmath,amssymb,amsfonts,amscd}
%%\usepackage{sectsty} % Enables custom section titles
%%\allsectionsfont{\usefont{OT1}{phv}{b}{n}} % Change the font of all section commands
%
%%\usepackage{fancyhdr} % Needed to define custom headers/footers
%%\usepackage{lastpage} % Used to determine the number of pages in the document (for "Page X of Total")
%%\usepackage{tikz}
%%\usetikzlibrary{calc,patterns,angles,quotes}
%%\usetikzlibrary{shapes.geometric, arrows}
%%\usepackage[abs]{overpic}
%%\usepackage{verbatim,color}
% 
%%\usepackage{adjustbox}
%%\usepackage{lettrine} % Package to accentuate the first letter of the text
%%\newcommand{\initial}[1]{ % Defines the command and style for the first letter
%%\lettrine[lines=3,lhang=0.3,nindent=0em]{
%%\color{DarkGoldenrod}
%%{\textsf{#1}}}{}}
%%---------------------------------------------------------------
%%\usepackage{titling} % Allows custom title configuration
%%
%%\newcommand{\HorRule}{\color{DarkGoldenrod} \rule{\linewidth}{1pt}} % Defines the gold horizontal rule around the title
%%
%% 
%
%%\usepackage{bm}
%
%%\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
%%\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
%%\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
%%\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
%%\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
%%\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
%%\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
%%\makeatother
%
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{remarks}{Remarks}
%\newtheorem{definition}{Definition}
%\newtheorem{assumption}{Assumption}
%\newtheorem{remark}{Remark}
%\newtheorem{problem}{Problem}
%\newtheorem{algoritm}{Alogrithm}
%\newtheorem{condition}{Condition}
%%---------------------------------------------------------------
%%\usepackage{enumitem}
%\numberwithin{figure}{section}
%\usepackage{graphicx}
%\usepackage{caption,subcaption}
%\usepackage{subfig}    
%\usepackage{float}
%\usepackage{subfig}
%\usepackage{epstopdf}
%\epstopdfsetup{update} %
%%\usepackage{cleveref}
%%\usepackage{subfig}
%\usepackage{cite}
%\usepackage{upgreek}
%
%\usepackage{cuted}
%\setlength\stripsep{3pt plus 1pt minus 1pt}
%
%
%%\DeclareMathOperator*{\minimize}{minimize}
%%\typeout{pdfcompresslevel=\the\pdfcompresslevel}
%%\typeout{pdfobjcompresslevel=\the\pdfobjcompresslevel}
%%\typeout{pdfminorversion=\the\pdfminorversion}
%%\pdfcompresslevel=9
%%\pdfminorversion=5
%%\pdfobjcompresslevel=2
%
\usepackage{ragged2e}


